ControlDreamer: Blending Geometry and Style in Text-to-3D

Recent advancements in text-to-3D generation have significantly contributed to the automation and democratization of 3D content creation. Building upon these developments, we aim to address the limitations of current methods in blending geometries and styles in text-to-3D generation. We introduce multi-view ControlNet, a novel depth-aware multi-view diffusion model trained on generated datasets from a carefully curated text corpus. Our multi-view ControlNet is then integrated into our two-stage pipeline, ControlDreamer, enabling text-guided generation of stylized 3D models. Additionally, we present a comprehensive benchmark for 3D style editing, encompassing a broad range of subjects, including objects, animals, and characters, to further facilitate research on diverse 3D generation. Our comparative analysis reveals that this new pipeline outperforms existing text-to-3D methods as evidenced by human evaluations and CLIP score metrics. Project page: https://controldreamer.github.io

==> Contents/backup.tex <==
%%%%% Figure  2 %%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{Figures/save_fig_new.pdf} 
\caption{Results from generating various stylized 3D models using style prompts, based on a source NeRF created from a geometry prompt. Our ControlDreamer (a) aligns various styles on the source geometry, while the baseline (b) suffers artifacts due to misalignment of style and geometry.}
\label{fig:fig2}
\vspace{-0.5em}
\end{figure}

 In the second stage, we found that pre-trained MVDream model encounters difficulties in aligning textures with the initially generated geometrical structures, resulting in noticeable artifacts as represented in Fig. \ref{fig:fig2} (b). 


 \section{Limitations and Future Works}
While ControlDreamer excels in generating stylized 3D models, it faces several limitations. Errors in pre-trained depth estimators can cause hole artifacts from the geometry stage to persist in the style stage. Another constraint is our experiment's 256x256 resolution limit, due to MVDream's training at this resolution. Integrating models like SDXL \cite{podell2023sdxl}, trained on 1024x1024 images, could be a solution for higher-resolution outcomes. Future work will likely focus on developing an image-conditioned MV-ControlNet and exploring data scaling strategies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\centering
\includegraphics[width=\linewidth]{Figures/abl_controlnet.pdf} 
\caption{The left plot illustrates the 3D model generation results at 45 degrees and 135 degrees under various input conditions. On the right, (a) demonstrates the refinement using Magic3D, and (b) highlights the results achieved with our ControlDreamer.}
\label{fig:abl_control}
\end{figure}


\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{Figures/multi_sources.pdf} 
\caption{The left column displays an array of initial 3D models. From each initials, multiple styles are applied to create 3D models. Utilizing a two-stage pipeline, this process generates customized 3D models with a variety of geometries, including samurai, Mr. Bean, stone bust, and a Messi figure, and styles including Iron Man, Captain America, and Superman.
}
\label{fig:multi_sources}
\end{figure*}
%%%%%%%%%%%%%%%


==> Tabs/tab2.tex <==
\begin{table*}[t!]
\centering
\caption{Results of evaluations of the directional CLIP similarity on five different categories.}
\label{tab:dir_clip}
{\resizebox{\textwidth}{!}
{\begin{tabular}{cccccc}
\hline
    \toprule
    Domain & Animals & Characters & Foods & General & Objects \\
    \midrule
    Magic3D & 0.218 $\pm$ 0.11 & 0.280 $\pm$ 0.12  & 0.236 $\pm$ 0.11 & 0.247 $\pm$ 0.11 & 0.217 $\pm$ 0.06 \\
    Fantasia3D & 0.191 $\pm$ 0.11 & 0.250 $\pm$ 0.09  & 0.256 $\pm$ 0.09 & 0.240 $\pm$ 0.09 & 0.208  $\pm$ 0.08 \\
    ProlificDreamer & 0.224 $\pm$ 0.09 & 0.265 $\pm$ 0.09  & 0.239 $\pm$ 0.10 & 0.231 $\pm$ 0.10 & 0.163 $\pm$ 0.07 \\
    MVDream 2-stage & 0.160 $\pm$ 0.09 & 0.235 $\pm$ 0.12  & 0.150 $\pm$ 0.09 & 0.211 $\pm$ 0.12 & 0.122 $\pm$ 0.08 \\
    \midrule
    ControlDreamer & \textbf{0.241 $\pm$ 0.11} & \textbf{0.353 $\pm$ 0.11}  & \textbf{0.270 $\pm$ 0.09} & \textbf{0.341 $\pm$ 0.08} & \textbf{0.255 $\pm$ 0.08} \\
    \bottomrule
\end{tabular}}}
\end{table*} 

% Magic3D \cite{lin2023magic3d} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\
% ProlificDreamer \cite{wang2023prolificdreamer} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\
% Fantasia3D \cite{chen2023fantasia3d} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\
    
% Two-Stage MVDream \cite{shi2023mvdream} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\

==> Tabs/tab3.tex <==
\begin{table*}[t!]
\centering
\caption{Additional results of evaluations of the CLIP similarity on five different categories.}
\label{tab:clip_eval}
{\resizebox{\textwidth}{!}
{\begin{tabular}{cccccc}
\hline
    \toprule
    Domain & Animals & Characters & Foods & General & Objects \\
    \midrule
    Magic3D & 0.165 $\pm$ 0.07 & 0.232 $\pm$ 0.04  & 0.182 $\pm$ 0.06 & 0.196 $\pm$ 0.07 & 0.150 $\pm$ 0.07 \\
    Fantasia3D & 0.163 $\pm$ 0.06 & 0.216 $\pm$ 0.04  & 0.179 $\pm$ 0.04 & 0.204 $\pm$ 0.09 & 0.127  $\pm$ 0.10 \\
    ProlificDreamer & 0.172 $\pm$ 0.06 & 0.234 $\pm$ 0.03  & 0.215 $\pm$ 0.05 & 0.205 $\pm$ 0.07 & 0.131 $\pm$ 0.07 \\
    MVDream 2-stage & 0.183 $\pm$ 0.05 & 0.255 $\pm$ 0.04  & 0.179 $\pm$ 0.03 & 0.211 $\pm$ 0.05 & 0.103 $\pm$ 0.05 \\
    \midrule
    ControlDreamer & \textbf{0.195 $\pm$ 0.08} & \textbf{0.272 $\pm$ 0.05}  & \textbf{0.179 $\pm$ 0.05} & \textbf{0.220 $\pm$ 0.08} & \textbf{0.129 $\pm$ 0.08} \\
    \bottomrule
\end{tabular}}}
\end{table*} 

% Magic3D \cite{lin2023magic3d} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\
% ProlificDreamer \cite{wang2023prolificdreamer} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\
% Fantasia3D \cite{chen2023fantasia3d} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\
    
% Two-Stage MVDream \cite{shi2023mvdream} & 0.27 \pm 0.09 & 0.35 \pm 0.11  & 0.35 \pm 0.11 & 0.27 \pm 0.09 & 0.27 \pm 0.09 \\
